Multi-task Learning for Identification of Porcelain in Song and Yuan Dynasties

Chinese porcelain holds immense historical and cultural value, making its accurate classification essential for archaeological research and cultural heritage preservation. Traditional classification methods rely heavily on expert analysis, which is time-consuming, subjective, and difficult to scale. This paper explores the application of DL and transfer learning techniques to automate the classification of porcelain artifacts across four key attributes: dynasty, glaze, ware, and type. We evaluate four Convolutional Neural Networks (CNNs) - ResNet50, MobileNetV2, VGG16, and InceptionV3 - comparing their performance with and without pre-trained weights. Our results demonstrate that transfer learning significantly enhances classification accuracy, particularly for complex tasks like type classification, where models trained from scratch exhibit lower performance. MobileNetV2 and ResNet50 consistently achieve high accuracy and robustness across all tasks, while VGG16 struggles with more diverse classifications. We further discuss the impact of dataset limitations and propose future directions, including domain-specific pre-training, integration of attention mechanisms, explainable AI methods, and generalization to other cultural artifacts.

==> removed.tex <==
\section{Dataset}

Typical samples are shown in Fig \ref{tab:data}.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{data.png}
  \captionof{figure}{Typical Samples of Porcelain Dataset}
  \label{tab:data}
\end{figure}


DYNASTY

The Song dynasty represents the inaugural golden age in the history of Chinese porcelain. Notable ceramic productions from this era encompass several distinguished ware systems: the Ding ware system, known for its white porcelain; the Jun ware system, which produced both white porcelain and underglaze-coloured porcelain; the Yaozhou ware system, recognized for its red and blue variegated glazes; the Yue ware and Longquan ware system, which specialized in celadon production in the southern regions; and the Black porcelain system, which crafted black porcelain and various black variegated glazes. Furthermore, the Song Imperial court undertook the establishment of Ru official ware, Jun official ware, Bianjing official ware, "Brother ware" and so on\cite{Shi2005Encyclopedia}.

The Yuan dynasty represented both the continuation and evolution of the Song dynasty's porcelain industry. Yuan-era porcelains occupied a transitional position between the peaks of the Song and Ming-Qing eras. On one hand, several celebrated Song wares - including Cizhou, Jingdezhen, and Longquan - maintained traditional production, particularly the signature green and white Longquan glazes which saw increasing scale. Conversely, towards the late Yuan period, the Jingdezhen wares pioneered novel glaze types such as blue-and-white, glazed red, cobalt blue, copper red, and pebble-white. These technical breakthroughs laid the groundwork for Jingdezhen's emergence as the premier centre of Chinese porcelain manufacture.\cite{Shi2005Encyclopedia}.

WARE

Based on the above reasons, this paper focuses on the selection of the dataset on the Song and Yuan dynasties, to provide possibilities and foundations for future research combining the Ming and Qing dynasties (another peak period of ancient Chinese porcelains). The data set also includes porcelains originating from ten different ware sites, distributed throughout the northern and southern regions of China (Fig \ref{tab:map}). These include the Ding ware produced in Hebei province, Ru and Junware produced in Henan, the Peng ware of Shanxi, as well as the celebrated Longquan ware of Zhejiang, the Linchuan, Xianghu and Jizhou wares of Jiangxi Province \cite{China1980}. Additionally, the dataset includes Geware, which precise ware sites remain undiscovered to the present day. The ten wares were chosen based partly on the quantity available collected from the National Palace Museum, but mainly due to their status, The Five Great Wares(Ding, Ru, Jun, Guan, and Ge ware) which produced Chinese porcelains during the Song dynasty \cite{rastelli2016concept}, Ding ware is characterized by its thin, white or greyish body and a nearly transparent white-tinted glaze \cite{rawson1984chinese}. The distinctive characteristic of Jun ware is its glaze colour, featuring glazes that range from blue to purple, sometimes exhibiting subtle white suffusions \cite{medley1976chinese}. Ge ware exhibits significant morphological and stylistic correlations with Guan ware, particularly in their characteristic crackle glaze effects. While classified within the broad celadon grouping, the glaze colour ranges from cream to ivory, presenting gradations toward grey or brownish tones, with little green in it \cite{vainker1991chinese}. Ru ware is distinguished by its characteristic pale 'duck-egg' blue glaze, Despite its minimalist aesthetic, this ware exhibits subtle chromatic variations, extending its palette to include subdued celadon green hues\cite{ru2017}.


GLAZE

In traditional identification, the quality of the glaze primarily relies on visual inspection. Experts evaluate the glaze based on various factors, including its colour, texture, brightness, transparency, and the size and distribution of air bubbles beneath the surface, ultimately drawing conclusions based on these observations. Colour is a significant indicator in glaze identification, as the mineral pigments in porcelain influence its hue. Even transparent glazes exhibit subtle colours, such as moon-white, bluish-white, or yellowish-green. For archaeological porcelains, completely colourless and transparent glazes are not found \cite{MaoXiaohu2016AncientCeramicsIdentification}.

The Song Sancai is a continuation of the Tang Sancai production, the Song Sancai was made in the Song Dynasty, and most of the porcelain fired are incense-burners, pillows, plates, washes, and other utility artifacts. The glaze colours are mostly yellow, green, white and brown. Fig \ref{tab:glaze} shows seven different glaze colours from the porcelain dataset.



TYPE

The porcelain industry developed and flourished in the Song dynasty. In order to meet the needs of all classes of people's material life, different wares around China burned abundant types of porcelain, such as bowls, plates, vases, saucers, washers, stoves, pillows, etc. These variations were closely tied to their intended use, including wine objects such as cups, storage containers like jars and pots, eating objects such as plates and bowls, and decorative display objects like vases  \cite{1982HistoryOfChineseCeramics}.

Each type of porcelain features a variety of forms. Craftsmen employed thick and thin lines, straight and curved shapes, and long and short contours. These different external outlines were combined to create forms that were both practical and beautiful, representing distinct characteristics of their respective times \cite{2015HistoryOfChineseCeramicsIdentification}. Fig \ref{tab:type} shows twelve different types from the porcelain dataset.


Using vases as an example, these artifacts exhibit a wide variety of styles, including the jade pot spring vase, plum vase, flat-bellied vase, melon prism vase, and gourd vase. Most variations in vase shapes were seen in the mouth, neck, and abdomen \cite{1982HistoryOfChineseCeramics}. They can be broadly categorized into two categories: one featuring a long and elegant body, and the other characterized by a short and stable form. However, slender shapes were more commonly found. Fig \ref{tab:vase} shows the vase type from the Song Dynasty of the dataset. We applied the edge-detection pipeline to highlight the edges of the object (a vase), the background of the image is cleanly separated, providing a clear visualization of the contours. This process is particularly effective for analyzing structural features, such as patterns, cracks, or boundaries in objects, as demonstrated in the vase. The Ding white vases exhibit elongated, slender forms. These shapes emphasize elegance and simplicity. Many Guan and Longquan celadon vases have more rounded designs, demonstrating a focus on symmetry and volume. 


\subsection{MultiTask Learning Framework}

\subsubsection{ResNet50}
We used a pre-trained ResNet50 by removing the top classification layers and freezing the weights. We then added task-specific convolutional layers for each classification task (dynasty, ware, glaze, type). This structure allows each task to learn its own features from the shared feature map. Subsequently, four fully connected layers were applied to produce outputs for each classification task. The ResNet50 structure is shown in Figure \ref{tab:resnet}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{resnet.png}
\caption{ResNet50 Structure of the Multi-Task Model}
\label{tab:resnet}
\end{figure}

Task-specific convolutional layers were added on top of the shared ResNet50 features to allow each task to learn its distinctive patterns from the shared feature space. Each task (dynasty, ware, glaze, type) has its convolutional layer block. These blocks consist of a sequence of operations aimed at refining the shared features into task-specific features. The sequence was as follows:
\begin{itemize}
\item \textbf{Convolutional Layer}\\
We applied a 2D convolution operation with 512 output channels, a kernel size of 3, and a padding of 1. This layer transformed the shared features into task-specific features.
This transformation captures spatial hierarchies relevant to each specific task.
\item \textbf{Batch Normalization}\\
Batch normalization normalized the outputs of the convolutional layer to accelerate training and improve stability. It helped to maintain the mean output close to 0 and the output standard deviation close to 1.
\item \textbf{ReLU Activation}\\
We applied a Rectified Linear Unit (ReLU) activation function, introducing non-linearity into the model, which helped to learn complex patterns.
\item \textbf{Adaptive Average Pooling}\\
This layer reduced the spatial dimensions of the feature map to 1x1, effectively summarizing the feature map into a single value per channel. This operation maked the output invariant to spatial transformations.
\end{itemize}

\subsubsection{MobileNetV2}
The MobileNetV2-based model followed a similar structure to the ResNet50-based model, with task-specific convolutional layers and fully connected layers added on top of the shared features. The MobileNetV2 structure is shown in Figure \ref{tab:mobilenet}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{mibilenetv2.png}
\caption{MobileNetV2 Structure of the Multi-Task Model}
\label{tab:mobilenet}
\end{figure}

\subsubsection{VGG16}
The VGG16-based model followed a structure where task-specific convolutional layers and fully connected layers were added on top of the shared features extracted by the pre-trained VGG16 model. The VGG16 structure is shown in Figure \ref{tab:vgg16}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{vgg16.png}
\caption{VGG16 Structure of the Multi-Task Model}
\label{tab:vgg16}
\end{figure}

\subsubsection{InceptionV3}
We used a pre-trained InceptionV3 by removing the top classification layers and freezing the weights. We then added task-specific fully connected layers for each classification task (dynasty, ware, glaze, type). This structure allows each task to learn its features from the shared feature map. Subsequently, four fully connected layers were applied to produce outputs for each classification task.

Due to the presence of the auxiliary classifier in InceptionV3, we did not add task-specific convolutional layers. Instead, the auxiliary classifier helps improve the learning process by providing an additional gradient signal. Each task (dynasty, ware, glaze, type) has its own fully connected layer. The InceptionV3 structure is shown in Figure \ref{tab:inception3}.


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{inceptionv3.png}
\caption{InceptionV3 Structure of the Multi-Task Model}
\label{tab:inception3}
\end{figure}

